Scene Perceived Image Perceptual Score (SPIPS): combining global and local perception for image quality assessment

The rapid advancement of artificial intelligence and widespread use of smartphones have resulted in an exponential growth of image data, both real (camera-captured) and virtual (AI-generated). This surge underscores the critical need for robust image quality assessment (IQA) methods that accurately reflect human visual perception. Traditional IQA techniques primarily rely on spatial features - such as signal-to-noise ratio, local structural distortions, and texture inconsistencies - to identify artifacts. While effective for unprocessed or conventionally altered images, these methods fall short in the context of modern image post-processing powered by deep neural networks (DNNs). The rise of DNN-based models for image generation, enhancement, and restoration has significantly improved visual quality, yet made accurate assessment increasingly complex. To address this, we propose a novel IQA approach that bridges the gap between deep learning methods and human perception. Our model disentangles deep features into high-level semantic information and low-level perceptual details, treating each stream separately. These features are then combined with conventional IQA metrics to provide a more comprehensive evaluation framework. This hybrid design enables the model to assess both global context and intricate image details, better reflecting the human visual process, which first interprets overall structure before attending to fine-grained elements. The final stage employs a multilayer perceptron (MLP) to map the integrated features into a concise quality score. Experimental results demonstrate that our method achieves improved consistency with human perceptual judgments compared to existing IQA models.

==> figs/framework.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/workflow.png}
    \caption{framework.
    }
    \label{fig:framework}
\end{figure*}


==> sec/0_abstract.tex <==
\begin{abstract}\vspace{-10pt}
   The rapid proliferation of smartphones and advancements in AI have led to an exponential increase in both real (camera-captured) and virtual (AI-generated) image data. This surge highlights the urgent need for a comprehensive image quality assessment method that aligns with human visual perception. Traditional approaches primarily focus on detecting artifacts by extracting spatial features such as signal-to-noise ratio, local structural distortions, and local texture distortions. While these methods are generally effective for raw images or those processed using traditional techniques, the emergence of deep neural networks (DNNs) has transformed image post-processing. With the development of numerous models for image generation, enhancement, and restoration, image quality has improved significantly, but assessing it has become considerably more challenging.

   Researchers have extensively explored deep learning-based image quality assessment. One widely adopted method in academia is LPIPS (Learned Perceptual Image Patch Similarity); however, discrepancies remain between LPIPS and other image quality assessment approaches. LPIPS is characterized by several key features:  

   \begin{itemize}
       \setlength\itemsep{0pt}
       \item A dedicated image dataset is collected specifically for image quality assessment.  
       \item Only the feature data from the initial layers of the backbone model are utilized, based on the assumption that these layers capture general features while deeper layers may introduce bias.  
       \item The assessment is conducted on image patches rather than the entire image.  
   \end{itemize}
   These characteristics indicate that LPIPS primarily focuses on evaluating the quality of image details.

   Building on these characteristics of LPIPS and our observation that the high-level features of the backbone model often capture the semantic information of an image scene, we propose a multi-channel feature analysis and transformation model. This model analyzes features within the same channel to compute spatial correlations and examines relationships between features of different channels to assess the connection between low-level and high-level features. By integrating these analyses, the model provides a more comprehensive evaluation of both image content and details, aligning with the human visual perception process, which first captures global structure before focusing on finer details. The final MLP layer maps the extensively analyzed features into a highly condensed quality score. In the experimental section, we will compare the performance of our model with state-of-the-art (SOTA) methods.
\\\vspace{-25pt}
\end{abstract}
